Mass-spectrometry of single mammalian cells quantifies proteome heterogeneity during cell differentiation

Cellular heterogeneity is important to biological processes, including cancer and development. However, proteome heterogeneity is largely unexplored because of the limitations of existing methods for quantifying protein levels in single cells. To alleviate these limitations, we developed Single Cell ProtEomics by Mass Spectrometry (SCoPE-MS), and validated its ability to identify distinct human cancer cell types based on their proteomes. We used SCoPE-MS to quantify over a thousand proteins in differentiating mouse embryonic stem (ES) cells. The single-cell proteomes enabled us to deconstruct cell populations and infer protein abundance relationships. Comparison between single-cell proteomes and transcriptomes indicated coordinated mRNA and protein covariation. Yet many genes exhibited functionally concerted and distinct regulatory patterns at the mRNA and the protein levels, suggesting that post-transcriptional regulatory mechanisms contribute to proteome remodeling during lineage specification, especially for developmental genes. SCoPE-MS is broadly applicable to measuring proteome configurations of single cells and linking them to functional phenotypes, such as cell type and differentiation potentials.

==> Figure_Captions.tex <==
%\include{Macros_Cell} \begin{document}
\section*{Figure Captions}

%\newcounter{figs} \addtocounter{figs}{1}

\begin{figure}[h!]
\caption{ \concept } 
\label{concept}
\end{figure}
\vspace{1cm} 



\begin{figure}[h!]
\caption{ \prot } 
\label{prot}
\end{figure}
\vspace{1cm} 

\begin{figure}[h!]
\caption{ \pca } 
\label{pca}
\end{figure}
\vspace{1cm} 




\begin{figure}[h!]
\caption{ \rnaProt } 
\label{rnaProt}
\end{figure}
\vspace{1cm} 
\newpage 

\setcounter{figure}{0} 

%
%\newpage       
%\setcounter{figure}{0}      
%\renewcommand{\thefigure}{ S\arabic{figure}}



%\begin{figure}[h!]
%\caption{ \RPLphospho } 
%\label{RPLphospho}
%\end{figure}
%\vspace{1cm} 




%
%\begin{figure}[h!]
%\caption{ {\bf Experimental validation of \name by UPS spike-in} \\
%{\bf A}, Schematic diagram of the experiment used to evaluate \name. We prepared a gold standard of proteins from the dynamic universal proteomics standard (UPS2) whose cysteines were covalently modified either with iodoacetamide or with vinylpyridine. Upon digestion, these modified UPS proteins generate many shared peptides (peptides not containing cysteine) and a few unique peptides (peptides containing cysteine). The modified UPS2 proteins were mixed with one another at known ratios ($n$), digested and quantified by MS. The ratios between the proteins that \name inferred from the MS data ($\hat n$) were compared with the mixing ratios. \\
% {\bf B}, The ratios \emph{between} the acetylated isoforms of UPS2 inferred by \name ($\hat n$, y-axis)  accurately reflect the mixing ratios ($n$, x-axis). \\
% {\bf C}, Comparison of the error in \name inferences and inferences based on the intensities of unique peptides.         
%}
%\label{ups}
%\end{figure}
%\vspace{1cm} 




%
%\begin{figure}[h!]
%\caption{ {\bf Validation of \name based on external standards for histone 3 and its PTMs} \\
%{\bf A}, The fractional site occupancies for histone 3 PTMs were estimated across a set of perturbations from SRM with MasterMix external standards with known concentrations \citep{}. These estimates were compared to the corresponding fractional site occupancies inferred by \name \emph{only} from the relative quantification, without using the MasterMix concentrations. The good agreement of the estimates validated the ability of \name to infer the ratios \emph{between} different isoforms. Different colors correspond to different PTMs and each circle is a condition/treatment. \\
% %{\bf B}, Comparison of mixing ratios ($n$) and ratios inferred by \name ($\hat n$). \\
% %{\bf C}, Comparison of the error in \name inferences and inferences based on the intensities of unique peptides.         
%}
%\label{h3}
%\end{figure}
%\vspace{1cm} 






%\begin{figure}[h!]
%\caption{ {\bf Validation of \name inference based only on shared peptides} \\
%{\bf A-B}, Evaluation of the inference accuracy by \name on simulated data as a function of the measurement noise. Peptide data were simulated from known ``gold-standard'' protein levels and based on system (1); see \supp. Protein levels for proteins having only shared peptides were inferred by \name from the simulated data and compared to the gold-standard; the accuracy is evaluated either by fractional difference (A) or by correlation (B). \\    
%{\bf C-D}, Proteins levels ($\mathbf {p}_{i}^S$) inferred \emph{only} from shared peptides accuretly correspond to ``gold standard'' levels ($\mathbf {p}_{i}^U$) estimated \emph{only}  from unique peptides; the accuracy is evaluated either by fractional difference (C) or by correlation (D) $\langle \mathbf {p}_{i}^S, \mathbf {p}_{i}^U \rangle$. \\
%{\bf E}, Analogous analysis as in (C) but applied to a mouse SILAC dataset.         
%}
%\label{shared}
%\end{figure}
%\vspace{1cm}




% Quantification of phosphorylated, acetylated and ubiqutylated isoforms

%\ssecc{Figure 5: Application to data from serial PTM enrichment}

%\end{document}














